Direct photon calculations in heavy-ion collisions at s(NN)**1/2 = 62.4 - 200 AGeV in a (3+1) dimensional hybrid approach

Direct photon spectra from central Au+Au- and Cu+Cu-collisions at sqrt(s_NN) = 62.4, 130 and 200 AGeV are calculated within the microscopic transport model UrQMD and a micro+macro hybrid model. In the latter approach, the high-density part of the transport evolution is replaced by an ideal 3+1-dimensional hydrodynamic calculation. We study the impact of viscosity and full local thermalization and compare the calculations to measurements obtained by the PHENIX collaboration. We find a reasonable agreement with the experimental data for calculations involving a Quark-Gluon-Plasma phase.

==> fitresults.tex <==
 \begin{tabular}{l|l|l|c|r@{.}l@{$\pm$}r@{.}l|r@{.}l@{$\pm$}r@{.}l|r@{.}l}
  System & $\sqrt{s_{\sf NN}}$ & EoS & centrality & \multicolumn{4}{c|}{$T_{\rm slope}~[$MeV$]$} & \multicolumn{4}{c|}{$A~[$GeV$^{-2}]$} & \multicolumn{2}{c}{$\chi^2$/d.o.f.} \\ \hline
  Au+Au & 200 & \color{red}Transport     & 00\%-20\% & 232&5 & 9&8 & 1&65 & 0&48 & 0&041 \\
  Au+Au & 200 & \color{blue}HG-EoS       & 00\%-20\% & 246&7 & 8&6 & 3&63 & 0&83 & 0&025 \\
  Au+Au & 200 & \color{orange}$\chi$-EoS & 00\%-20\% & 261&9 & 8&7 &10&13 & 2&05 & 0&020 \\
  Au+Au & 200 & \color{violett}BM-EoS    & 00\%-20\% & 251&4 & 9&7 &16&37 & 4&03 & 0&029 \\
  Au+Au & 200 & Transport & 20\%-40\% & 237&3 &12&1 & 0&38 & 0&13 & 0&057 \\
  Au+Au & 200 & HG-EoS    & 20\%-40\% & 243&4 & 8&3 & 1&32 & 0&30 & 0&025 \\
  Au+Au & 200 & $\chi$-EoS& 20\%-40\% & 253&0 & 8&0 & 4&11 & 0&82 & 0&020 \\
  Au+Au & 200 & BM-EoS    & 20\%-40\% & 240&6 & 9&0 & 7&61 & 1&90 & 0&030 \\\hline
  Au+Au & 130 & Transport & 00\%-20\% & 232&5 & 9&1 & (9&87 & 2&67)$\cdot 10^{-2}$ & 0&035 \\
  Au+Au & 130 & Transport & 20\%-40\% & 257&2 &11&3 & (5&48 & 1&50)$\cdot 10^{-3}$ & 0&036 \\
  Au+Au & 130 & HG-EoS    & 00\%-20\% & 246&3 & 8&5 & 3&42 & 0&66 & 0&024 \\
  Au+Au & 130 & HG-EoS    & 20\%-40\% & 242&4 & 7&6 & 1&26 & 0&26 & 0&021 \\
  Au+Au & 130 & $\chi$-EoS& 00\%-20\% & 261&2 & 8&5 & 9&67 & 1&93 & 0&019 \\
  Au+Au & 130 & $\chi$-EoS& 20\%-40\% & 252&7 & 7&9 & 4&01 & 0&80 & 0&019 \\
  Au+Au & 130 & BM-EoS    & 00\%-20\% & 250&2 & 9&6 &15&84 & 3&88 & 0&039 \\
  Au+Au & 130 & BM-EoS    & 20\%-40\% & 240&6 & 8&8 & 7&46 & 1&82 & 0&029 \\ \hline
  Au+Au & 62.4& Transport & 00\%-20\% & 242&1 &13&5 &(5&29 & 1&95)$\cdot 10^{-2}$ & 0&066 \\
  Au+Au & 62.4& Transport & 20\%-40\% & 232&8 & 9&4 &(4&18 & 1&16)$\cdot 10^{-3}$ & 0&038 \\
  Au+Au & 62.4& HG-EoS    & 00\%-20\% & 247&3 & 8&1 & 3&19 & 0&67 & 0&022 \\
  Au+Au & 62.4& HG-EoS    & 20\%-40\% & 245&8 & 8&0 & 1&21 & 0&26 & 0&022 \\
  Au+Au & 62.4& $\chi$-EoS& 00\%-20\% & 261&8 & 8&2 & 9&24 & 1&78 & 0&018 \\
  Au+Au & 62.4& $\chi$-EoS& 20\%-40\% & 253&9 & 7&7 & 3&82 & 0&73 & 0&018 \\
  Au+Au & 62.4& BM-EoS    & 00\%-20\% & 250&3 & 9&5 &15&13 & 3&65 & 0&028 \\
  Au+Au & 62.4& BM-EoS    & 20\%-40\% & 240&8 & 8&6 & 7&33 & 1&74 & 0&028 \\ \hline
  Cu+Cu & 200 & HG-EoS    & 00\%-20\% & 252&0 & 9&6 &(4&84 & 1&38)$\cdot 10^{-1}$ & 0&057 \\
  Cu+Cu & 200 & HG-EoS    & 20\%-40\% & 254&6 &13&2 &(1&61 & 0&62)$\cdot 10^{-1}$ & 0&103 \\
  Cu+Cu & 200 & $\chi$-EoS& 00\%-20\% & 251&5 & 7&3 & 1&77 & 0&39 & 0&033 \\
  Cu+Cu & 200 & $\chi$-EoS& 20\%-40\% & 242&9 & 7&0 &(7&25 & 1&63)$\cdot 10^{-1}$ & 0&036 \\
  Cu+Cu & 200 & BM-EoS    & 00\%-20\% & 237&7 & 7&8 & 3&61 & 0&94 & 0&047 \\
  Cu+Cu & 200 & BM-EoS    & 20\%-40\% & 229&2 & 7&5 & 1&60 & 0&43 & 0&051 \\\hline
  Cu+Cu & 130 & HG-EoS    & 00\%-20\% & 250&0 & 9&3 &(4&78 & 1&35)$\cdot 10^{-1}$ & 0&056 \\
  Cu+Cu & 130 & HG-EoS    & 20\%-40\% & 240&4 & 7&7 &(1&99 & 0&50)$\cdot 10^{-1}$ & 0&044 \\
  Cu+Cu & 130 & $\chi$-EoS& 00\%-20\% & 250&9 & 7&1 & 1&76 & 0&37 & 0&031 \\
  Cu+Cu & 130 & $\chi$-EoS& 20\%-40\% & 242&8 & 7&1 &(6&99 & 1&59)$\cdot 10^{-1}$ & 0&036 \\
  Cu+Cu & 130 & BM-EoS    & 00\%-20\% & 238&1 & 7&9 & 3&56 & 0&93 & 0&048 \\
  Cu+Cu & 130 & BM-EoS    & 20\%-40\% & 228&5 & 7&7 & 1&58 & 0&44 & 0&054 \\\hline
  Cu+Cu & 62.4& HG-EoS    & 00\%-20\% & 248&2 & 7&7 &(4&71 & 1&11)$\cdot 10^{-1}$ & 0&039 \\
  Cu+Cu & 62.4& HG-EoS    & 20\%-40\% & 242&8 & 6&9 &(1&87 & 0&41)$\cdot 10^{-1}$ & 0&034 \\
  Cu+Cu & 62.4& $\chi$-EoS& 00\%-20\% & 250&2 & 6&8 & 1&71 & 0&35 & 0&029 \\
  Cu+Cu & 62.4& $\chi$-EoS& 20\%-40\% & 241&7 & 6&3 &(6&71 & 1&37)$\cdot 10^{-1}$ & 0&029 \\
  Cu+Cu & 62.4& BM-EoS    & 00\%-20\% & 236&8 & 7&4 & 3&52 & 0&88 & 0&044 \\
  Cu+Cu & 62.4& BM-EoS    & 20\%-40\% & 227&0 & 6&7 & 1&62 & 0&40 & 0&042 \\ \hline
 \end{tabular}

